Data-driven polynomial ridge approximation using variable projection

Inexpensive surrogates are useful for reducing the cost of science and engineering studies involving large-scale, complex computational models with many input parameters. A ridge approximation is one class of surrogate that models a quantity of interest as a nonlinear function of a few linear combinations of the input parameters. When used in parameter studies (e.g., optimization or uncertainty quantification), ridge approximations allow the low dimensional structure to be exploited, reducing the effective dimension. We introduce a new, fast algorithm for constructing a ridge approximation where the nonlinear function is a polynomial. This polynomial ridge approximation is chosen to minimize least squared mismatch between the surrogate and the quantity of interest on a given set of inputs. Naively, this would require optimizing both the polynomial coefficients and the linear combination of weights; the latter of which define a low-dimensional subspace of the input space. However, given a fixed subspace the optimal polynomial can be found by solving a linear least-squares problem, and hence by using variable projection the polynomial can be implicitly found leaving an optimization problem over the subspace alone. We provide an algorithm that finds this polynomial ridge approximation by minimizing over the Grassmann manifold of low-dimensional subspaces using a Gauss-Newton method. We provide details of this optimization algorithm and demonstrate its performance on several numerical examples. Our Gauss-Newton method has superior theoretical guarantees and faster convergence than the alternating approach for polynomial ridge approximation earlier proposed by Constantine, Eftekhari, Hokanson, and Ward [https://doi.org/10.1016/j.cma.2017.07.038] that alternates between (i) optimizing the polynomial coefficients given the subspace and (ii) optimizing the subspace given the coefficients.

==> algorithm_old.tex <==

\section{Algorithm}
Solve the least squares ridge function approximation we use Gauss-Newton on the Grassmann manifold.
To simply state our algorithm, we first reformulate the objective function~(\ref{eq:opt})
to clearly expose the nonlinear least squares structure.
As $g$ is a polynomial on $\ma U^\trans \ve x$, we can write $g(\ma U^\trans \ve x_i)$ as the product
of a multivariate Vandermonde matrix $\ma V(\ma U)$ and the polynomial coefficients $\ve c$
\begin{equation}\label{eq:vdef}
	g(\ma U^\trans \ve x_i) = \sum_{j=1}^{m +p\choose p} c_i \prod_{k=1}^m [\ma U^\trans \ve x_i]^{[\ve \alpha_j]_k} = [\ma V(\ve U)\ve c]_i,
	\quad [\ma V(\ma U)]_{i,j} := \prod_{k=1}^m [\ma U^\trans \ve x_i]_k^{[\ve\alpha_j]_k}
\end{equation}
where $\lbrace \ve \alpha_j \rbrace_{j=1}^{m+p\choose p}$ is the set of all length $m$ multi-indices with non-negative entires
and a sum less than or equal to $p$.
With this compact expression for the values of the ridge function approximation, 
we can then restate the optimization problem~(\ref{eq:opt}) as
\begin{equation}\label{eq:optmat}
	\min_{\ve c \in \R^{{m +p\choose p}}, \ma U\in \mathbb{G}(m, \R^n)} \quad
	 \left\| 
		\ve f - \ma V(\ma U) \ve c
	\right\|_2^2,
	\qquad [\ve f]_i = f(\ve x_i).
\end{equation} 
Our approach for solving this optimization problem consists of two steps.
First, using Variable Projection we implicitly remove the polynomial coefficients $\ve c$ and obtain an expression for the Jacobian.
Then we use this Jacobian to compute the Gauss-Newton search direction
and use a line search along this trajectory through the space of Grassmann manifolds.
These two topics are addressed in the remainder of the section and we conclude with a discussion of the full algorithm. 


\subsection{Variable Projection}
The key insight for Variable Projection is that once the nonlinear parameter $\ma U$ is fixed, the linear variables are fixed.
Namely, given $\ma U$, the polynomial coefficients $\ve c$ are given by the pseudoinverse: $\ve c(\ma U) = \ma V(\ma U)^+ \ve f$.
Hence, the optimization problem~(\ref{eq:optmat}) can be restated over $\ma U$ by replacing $\ve c$ with its implicit solution:
\begin{equation}
	\min_{\ma U \in \mathbb{G}(m, \R^n)} \| \ve f - \ma V(\ma U) \ma V(\ma U)^+\ve f\|_2^2.
\end{equation}
Alternatively, we can write this optimization problem as over the projector $\ma P_{\ma V(\ma U)}^\perp$ 
onto the orthogonal complement of the range of $\ma V(\ma U)$
\begin{equation}
	\min_{\ma U \in \mathbb{G}(m, \R^n)} \| \ma P_{\ma V(\ma U)}^\perp \ve f\|_2^2.
\end{equation}
The primary contribution of Golub and Pereyra~\cite{GP73} reveals a formula 
for the derivative of the residual $\ve r(\ma U) = \ma P_{\ma V(\ma U)}^\perp \ve f$,
$\ten J(\ma U)\in \R^{N \times n\times m}$
\begin{equation}\label{eq:ten_J}
	[\ten J(\ma U)]_{\cdot, j,k} = -\left[
			\left(\ma P_{\ma V(\ma U)}^\perp \frac{\partial \ma V}{\partial [\ma U]_{j,k}} (\ma U) \  \ma V(\ma U)^-\right)
			+ 
			\left(\ma P_{\ma V(\ma U)}^\perp \frac{\partial \ma V}{\partial [\ma U]_{j,k}} (\ma U) \ \ma V(\ma U)^-\right)^\trans
		\right]\ve f,
\end{equation}
where $^-$ denotes a least squares pseudoinverse where $\ma V\ma V^-\ma V = \ma V$ and $\ma V\ma V^- = (\ma V\ma V^-)^\trans$.
The derivative of $\ma V$ above is
\begin{align*}
	\left[\frac{\partial \ma V}{\partial [\ma U]_{k,\ell}}(\ma U)\right]_{i,j} &= 
		%\frac{\partial}{\partial [\ma U]_{k,\ell}} \prod_{q=1}^n [\ma U^\trans \ve x_i]^{[\ve \alpha_j]_q}_q %\\
		 [\ve \alpha_j]_\ell [\ma U^\trans \ve x_i]_\ell^{[\ve \alpha_j]_\ell-1} [\ve x_i]_k
			 \prod_{\substack{q=1\\ q\ne \ell}}^n [\ma U^\trans \ve x_i]_q^{[\ve \alpha_j]_q}.
\end{align*}

From this Jacobian, the gradient is:
\begin{equation}
	\ve g(\ma U) = \sum_{i=1}^N [\ten J(\ma U)]_{i,\cdot,\cdot} [\ve r(\ma U)]_i.
\end{equation}


\subsection{Grassmann Optimization}
Compared to optimization on Euclidean space, 
optimization on the Grassmann manifold requires several modifications.
Here we follow the approach of Edelman, Arias, and Smith~\cite{EAS98}
parametrizing the Grassmann manifold by the matrix $\ma U$ with orthonormal columns.
This describes each element in the Grassmann manifold using more parameters than are necessary, 
but permits easier computation.
We first review Newton's method on the Grassmann manifold before 
describing the modifications for the Gauss-Newton on the Grassmann manifold.


The fundamental difference for optimization over Grassmann manifold compared to optimization over
Euclidean space is that optimization moves along geodesics in the Grassmann manifold.
If given a search direction $\ve d$ (say by the gradient) in Euclidean space, we would update the current estimate
$\ve x_0$ by $\ve x(t) = \ve x_0 + t \ve d$ where the step length $t$ is chosen to ensure convergence.
In contrast, on the Grassmann manifold, this trajectory with constant derivative is replaced by a geodesic.
Using Theorem~2.3 from~\cite{EAS98}, given the current estimate $\ma U_0$ and search direction $\ma \Delta$,
the equivalent trajectory starting from $\ma U(0) = \ma U_0$ and following tangent $\dma U(0) = \ma \Delta$ is 
\begin{equation}
	\ma U(t) = \ma U(0) \ma Z \cos (\ma \Sigma t) \ma Z^\trans + \ma Y \sin(\ma \Sigma t) \ma Z^\trans 
\end{equation}
where $\ma Y \ma \Sigma \ma Z^\trans = \ma \Delta$ is the short form singular value decomposition.
Using this formula, we can also define the gradient of the objective function
$\phi(\ma U) = \frac12 \| \ma P_{\ma V(\ma U)}^\perp \ve f\|_2^2$.
First, following~\cite[(2.52)\&(2.56)]{EAS98}, we define the derivatives of the objective function 
with respect to the parameter $\ma U$ as
\begin{align}
	[\phi_{\ma U}]_{i,j} &:= \frac{\partial \phi}{\partial [\ma U]_{i,j}} 
	& \phi_\ma U&\in \R^{n\times m} \\
	[\phi_{\ma U\ma U}]_{i,j,k,\ell} &:= \frac{\partial^2 \phi}{\partial [\ma U]_{i,j} \partial [\ma U]_{k,\ell}} 
	& \phi_\ma U&\in \R^{n\times m\times n \times m} 
\end{align} 
With these definitions, the gradient of $\phi$ on the Grassmann manifold is~\cite[(2.70)]{EAS98}
is the component of $\phi_\ma U$ orthogonal to $\ma U$
\begin{align}
	\nabla \phi = \phi_\ma U - \ma U \ma U^\trans \phi_\ma U = \ma P_{\ma U}^\perp \phi_\ma U.
\end{align}
The Hessian of $\phi$ on the Grassmann manifold is defined implicitly 
through its action on two test matrices $\ma \Delta_1$ and $\ma \Delta_2$ following~\cite[(2.71)]{EAS98}
\begin{equation}\label{eq:Hessian}
	\Hess \phi (\ma \Delta_1, \ma \Delta_2) = \sum_{i,j,k,\ell} [\phi_{\ma U\ma U}]_{i,j,k,\ell} [\ma \Delta_1]_{i,j} [\ma \Delta_2]_{k,\ell}
			- \trace (\ma \Delta_1^\trans \ma \Delta_2 \ma U^\trans \ma \phi_\ma U).
\end{equation}
With these definition, Newton's method searches along the direction $\ma \Delta = [\Hess \phi]^{-1}\nabla \phi$
tangent to the current estimate $\ma U$.
That is, we choose $\ma \Delta \in \R^{n\times m}$ such that:
\begin{equation}\label{eq:hessian}
	\begin{split}
		\Hess \phi(\ma \Delta, \ma X) &= -\langle \nabla \phi,\ma X\rangle 
		\qquad  \forall \ \ma X \text{ s.t. } \ma U^\trans\ma X = 0 \\
		\ma U^\trans \ma \Delta &= 0
	\end{split}	
\end{equation} 
where the inner product $\langle \cdot, \cdot\rangle$ on this space is~\cite[(2.69)]{EAS98}
\begin{equation}\label{eq:inner}
	\langle \ma X, \ma Y\rangle = \trace \ma X^\trans \ma Y = (\vectorize \ma X)^\trans (\vectorize \ma Y).
\end{equation}


\subsection{Ridge Approximation Properties}
The structure of the ridge function approximation makes optimization on the Grassmann manifold easy.
In particular, the second term of the Hessian~(\ref{eq:hessian}) vanishes as $\ma U^\trans \phi_\ma U=\ma 0$.
This result stems from the fact that $\ma U^\trans [\ten J(\ma U)]_{i,\cdot,\cdot}=\ma 0$ which, in itself, is also useful.

To prove this result, first note 
\begin{align*}
	\left[\ma U^\trans [\ten J(\ma U)]_{i,\cdot,\cdot}\right]_{j,k}\!\!
		&= \sum_\ell [\ma U]_{\ell,j} [\ten J(\ma U)]_{i,\ell,k} \\
		&= \!-\!\sum_{\ell} [\ma U]_{\ell,j} \! \!\left[  
			\ma P_{\ma V(\ma U)}^\perp \frac{\partial \ma V(\ma U)}{\partial [\ma U]_{\ell,k}}
				\ma V(\ma U)^{-1} \ve f
			\!+\! \ma V(\ma U)^{-\!\trans} \frac{\partial \ma V(\ma U) }{\partial [\ma U]_{\ell,k}}^\trans \! \ma P_{\ma V(\ma U)}^\perp \ve f
		\right]_i 
\end{align*}
and by linearity we can take the sum inside each term, leaving
\begin{align*}
		= -\!\left[  
			\ma P_{\ma V(\ma U)}^\perp \! \left[ \sum_\ell [\ma U]_{\ell, j} \frac{\partial \ma V(\ma U)}{\partial [\ma U]_{\ell,k}} \right]
				\! \ma V(\ma U)^{-1} \ve f
			+ \ma V(\ma U)^{-\!\trans} \!
				\left[ \sum_\ell [\ma U]_{\ell, j} \frac{\partial \ma V(\ma U) }{\partial [\ma U]_{\ell,k}}^\trans\right]
		 \!\ma P_{\ma V(\ma U)}^\perp \ve f
		\right]_i\!.
\end{align*}
This interior sum results in matrix in the range of $\ma V(\ma U)$: 
\begin{align*}
	\left[\sum_\ell [\ma U]_{\ell,j} \frac{\partial \ma V(\ma U)}{\partial [\ma U]_{\ell,k}}\right]_{r,q}
		&= \sum_\ell [\ma U]_{\ell,j} [\ve \alpha_q]_k [\ma U^\trans\ve x_r]_k^{[\ve \alpha_q]_k -1} [\ve x_r]_\ell
			\prod_{\substack{s=1\\ s\ne k}}^n [\ma U^\trans \ve x_r]^{[\ve \alpha_q]_s}_s \\
		&= [\ve \alpha_q]_k [\ma U^\trans \ve x_r]^{[\ve \alpha_q]_k - 1}_\ell [\ma U^\trans \ve x_r]_j
			\prod_{\substack{s=1\\ s\ne k}}^n [\ma U^\trans \ve x_r]^{[\ve \alpha_q]_s}_s 
\end{align*}
Then since this matrix is in the range of $\ma V(\ma U)$, when multiplied by the orthogonal projector onto
the space perpendicular to $\Range \ma V(\ma U)$, it vanishes
\begin{equation}\label{eq:UJ}
	\ma U^\trans [\ten J(\ma U)]_{i,\cdot,\cdot}=\ma 0.
\end{equation}
The $\ma U^\trans \phi_\ma U$ term also vanishes since this is a linear combination of $\ma U^\trans [\ten J(\ma U)]_{i,\cdot,\cdot}$:
\begin{equation}\label{eq:Uphi}
	\ma U^\trans \phi_\ma U = \sum_{i} \ma U^\trans [\ten J(\ma U)]_{i,\cdot,\cdot} [\ve r(\ma U)]_i = \ma 0.
\end{equation}

\subsection{Grassmann Gauss-Newton}
Equipped with the special properties of the ridge function Jacobian from~(\ref{eq:UJ}) and~(\ref{eq:Uphi})
we now derive the Gauss-Newton method on the Grassmann manifold for this objective function.
First, using $\ma U^\trans \phi_\ma U = \ma 0$ to drop the second term in the Hessian~(\ref{eq:Hessian})
and expanding the inner product~(\ref{eq:inner}) the Newton step $\ma \Delta$ solves:
\begin{equation}\label{eq:Newton2}
	\begin{split}
		\sum_{i,j,k,\ell} [\phi_{\ma U\ma U}]_{i,j,k,\ell} [\ma \Delta]_{i,j} [\ma X]_{k,\ell} &= -(\vectorize \phi_{\ma U})^\trans (\vectorize \ma X)
		\qquad  \forall \ \ma X \text{ s.t. } \ma U^\trans\ma X = 0 \\
		\ma U^\trans \ma \Delta &= 0
	\end{split}	
\end{equation} 
The Gauss-Newton method replaces $\phi_{\ma U\ma U}$ with an approximation formed using the Jacobian:
\begin{equation}
	[\phi_{\ma U\ma U}]_{i,j,k,\ell} \approx \sum_{q} [\ten J(\ma U)]_{q,i,j} [\ten J(\ma U)]_{q,k,\ell}.
\end{equation}
With a little maneuvering, this expression can be rearranged to look like normal equations.
First, the left hand side of~(\ref{eq:Newton2}) can be rewritten with the Gauss-Newton Hessian approximation as 
\begin{equation}
	\sum_{i,j,k,\ell, q} [\ten J(\ma U)]_{q,i,j} [\ma \Delta]_{i,j} [\ten J(\ma U)]_{q,k,\ell} [\ma X]_{k,\ell}
		= (\vectorize \ma X)^\trans (\vectorize \ten J(\ma U))   (\vectorize \ten J(\ma U))^\trans (\vectorize \ma \Delta)
\end{equation}
where $\vectorize \ma X$ vectorizes matrices into a column vector 
and $\vectorize \ten J$ vectorizes a tensor into a matrix by flattening the last two indices.
Next, the right hand side of~(\ref{eq:Newton2}) can be rearranged to reveal the Jacobian tensor $\ten J(\ma U)$:
\begin{align*}
	(\vectorize \phi_\ma U)^\trans (\vectorize X) &= \trace \phi_\ma U^\trans \ma X 
		= \trace \left[ \sum_i \ma X^\trans[\ten J(\ma U)]_{i,\cdot,\cdot} [\ve r(\ma U)]_i \right] \\
		&= \sum_i (\vectorize \ten J(\ma U))^\trans (\vectorize \ma X) [\ve r(\ma U)]_i  = (\vectorize \ma X)^\trans (\vectorize \ten J(\ma U)) \ve r(\ma U)
\end{align*}
Combining these two results, we note that~(\ref{eq:Newton2}) is the normal equations stated in weak form:
\begin{equation}\label{eq:normal}
	(\vectorize \ma X)^\trans (\vectorize \ten J(\ma U)) (\vectorize \ten J(\ma U))^\trans (\vectorize \ma \Delta)
	\!=\! (\vectorize \ma X)^\trans (\vectorize \ten J(\ma u))\ve r(\ma U),  \ 
\end{equation}
for all $\ma X$ such that $\ma U^\trans \ma X = \ma 0$.

To convert~(\ref{eq:normal}) to a least squares problem,
 we first remove the constraint on $\ma X$ by adding a projector onto
the orthogonal complement of the range of $\ma U$:
\begin{equation}
	(\vectorize \ma P_\ma U^\perp \ma X)^\trans (\vectorize \ten J(\ma U))
	 (\vectorize \ten J(\ma U))^\trans ( \vectorize \ma \Delta)
	\!=\! (\vectorize \ma P_\ma U^\perp \ma X)^\trans (\vectorize \ten J(\ma u))\ve r(\ma U)
\end{equation}
for all $\ma X\in \R^{n\times m}$.
Transferring this projector onto $\vectorize \ten J(\ma U)$ it vanishes by~(\ref{eq:UJ})
\begin{align*}
	[(\vectorize \ma P_\ma U^\perp \ma X)^\trans (\vectorize \ten J(\ma U))]_{i}
	= \trace \ma X^\trans (\ma I - \ma U\ma U^\trans) [\ten J(\ma U)]_{i,:,:}
	= \trace \ma X^\trans [\ten J(\ma U)]_{i,\cdot,\cdot}
\end{align*}
Then, removing the normal equations, we seek to solve a constrained least squares problem
\begin{equation}
	\min_{\substack{\ma \Delta \in \R^{n\times m} \\ \ma U^\trans \ma \Delta = \ma 0}}
	\left\| \ve r(\ma U) + \vectorize \ten J(\ma U) \vectorize \ma \Delta\right\|_2
\end{equation}
or equivalently
\begin{equation}\label{eq:gnls}
	\min_{\substack{\ma \Delta \in \R^{n\times m} \\ \ma U^\trans \ma \Delta = \ma 0}} \left\|
		\ve r(\ma U) +
		\begin{bmatrix}
			[\ten J(\ma U)]_{\cdot,\cdot,1} &
			\ldots &
			[\ten J(\ma U)]_{\cdot,\cdot,n}
		\end{bmatrix}
		\begin{bmatrix}
			[\ma \Delta]_{\cdot,1} \\
			\vdots \\
			[\ma \Delta]_{\cdot,n}
		\end{bmatrix}
	\right\|_2
\end{equation}
The constraint can be equivalently be written in terms of the Kronecker product:
\begin{equation*}
	\ma U^\trans \ma \Delta = \ma 0 \quad  \Longleftrightarrow 
	\quad  (\ma I_n \otimes \ma U) \vectorize \ma \Delta = \ve 0.
\end{equation*}


The solution to~(\ref{eq:gnls}) is surprising easy to obtain using the pseudoinverse.
Noting from~(\ref{eq:UJ}), the matrix $\vectorize \ten J(\ma U)$ has a nontrivial nullspace.
\begin{align*}
	\left[ [\ten J(\ma U)]_{\cdot,\cdot, k} \ma U\right]_i = \sum_{j} [\ma U]_{j,\ell} [\ten J(\ma U)]_{i,j,k} = \ma 0.
\end{align*}
This nullspace contains the range of $\ma I_n \otimes \ma U$.
Hence if we choose $\ma \Delta$ to be 
\begin{equation}
	\vectorize \ma \Delta = \left( \vectorize \ten J(\ma U)\right)^+ \ve r(\ma U),
\end{equation}
$\ma \Delta$ will automatically satisfy the constraint $\ma U^\trans \ma \Delta =\ma 0$.


\subsection{Algorithm}
To obtain a convergent algorithm, we couple the Gauss-Newton search direction with a backtracking line search.

In practice it is necessary to choose a small backtracking acceptance parameter $\beta$, e.g., $\beta = 10^{-4}$.

\input{alg_main}

\jeffnote{TODO: Describe how efficiently implement Jacobian construction.}

\jeffnote{Do we want to prove the convergence of this algorithm?
	It should be straightforward following Nocedal and Wright, but we'll need to account for the rank-deficient Jacobian in Euclidean space
	(it is not rank-deficient restricted to the tangents on the Grassmann manifold).
}



==> fig_silhouet.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{groupplot}[
	group style = {group size = 2 by 1},
	width = 7cm,
	height = 5cm,
	ylabel = $f(\ve x)$
	]
	\nextgroupplot[xlabel=$\ve x_{21}$, title = {Coordinate Shadow Plot}]
	\addplot[black, only marks, mark size=0.5] table [x=xi, y=y] {fig_silhouet_data.dat}; 

	\nextgroupplot[xlabel=$\ma U^\trans \ve x$, title = {Subspace Shadow Plot}]
	\addplot[black, only marks, mark size=0.5] table [x=Ux, y=y] {fig_silhouet_data.dat};
	\addplot[colorbrewerA1, very thick] table [x=xfit, y=yfit] {fig_silhouet_fit.dat};
\end{groupplot}
\end{tikzpicture} \\
\begin{tikzpicture}
	\begin{axis}[
		width = 13cm,
		height = 3cm,
		xlabel = parameter $i$,
		ylabel = {$[\ma U]_i$},
		ymax = 0.6,
		ymin = -0.4,
		xmin = 0, 
		xmax = 98, 
		xtick = {1,10,20, ..., 90, 97},
		title = {Projection Weights}
		]
		\addplot[black, only marks, mark size = 1] table {fig_silhouet_U.dat};
		\addplot[black, thin, dashed] coordinates {(62.5, -1) (62.5, 1)};
		\node at (axis cs:50,0.6) [anchor=north] {\footnotesize design variables}; 
		\node at (axis cs:77,0.6) [anchor=north] {\footnotesize uncertain variables\phantom{g}}; 
	\end{axis}
\end{tikzpicture}

\caption{
	Two shadow plots show the response of $f(\ve x)$ to the projection
	of the input parameters $\ve x$ onto the subspace spanned by $\ma U$.
	Here, $f(\ve x)$ is a modified $p$-norm constraint agglomeration function
	from~\cite{SEQUOIA2017} where $\ve x\in \R^{97}$
	consists of $62$ design variables and $35$ uncertain variables.
	A polynomial ridge approximation with subspace dimension one
	and polnyomial degree seven was fit to $N=1000$ samples of this function
	and is shown as a red mark above.
	The bottom plot shows the weight attached to each parameter $\ve x$
	from the matrix $\ma U$.
	Looking down the direction of largest variation in a single coordinate on the left,
	no structure is apparent in $f(\ve x)$.
	However, looking along the direction $\ma U\in \R^{m\times 1}$
	reveals a one dimensional check-mark shaped function.
}
\label{fig:silhouet}
\end{figure}


==> intro_old.tex <==

\hrule

Inexpensive surrogates are key for reducing the cost of complex engineering problems.
For example, we may be given a function $f$ which maps a design parameterized by $m$-variables
$\ve x\in \set D \subset \R^m$ onto a particular quantity of interest, e.g., the thrust of a jet engine.
This function $f$ may be expensive to evaluate,
e.g., requiring the solution to a large partial differential equation model for each design $\ve x$.
As such, we may desire to replace this function $f$ by an inexpensive surrogate.
Although there are many forms this surrogate might take, 
here we choose to approximate $f$ by a polynomial $g$ that acts on a low-dimensional subspace
of the design variables:
\begin{equation}
	f(\ve x) \approx g(\ma U^\trans \ve x), \quad \text{where} \quad \ma U\in \R^{n\times m}, \quad \ma U^\trans \ma U = \ma I.
\end{equation}


When evaluating this function is expensive, 
Evaluating this function $f$ may be expensive, taking several hours and requiring the 


A prototypical example is maximizing the thrust of a jet engine.
Here, the engine is parameterized by $m$-variables $\ve x$ that reside in a design space $\set D\subset \R^m$
and the thrust of this design is given by the scalar function $f: \set D\to \R$.
Evaluating $f$ may be expensive, taking many hours as $f$ may require solving a partial differential equation,
and $f$ may contain nontrivial amounts of computational noise~\cite{MW11}.

This makes optimization of thrust expensive and, if derivative information is not available,
the computational noise might make finite difference approximations inpractical.
This motivates the construction of surrogates which are cheap to evaluate and have
accessible derivatives.
Although there are many forms for these surrogates, we choose our surrogate to be a 
\emph{ridge function}~\cite{CEW16}, where $f$ is approximated by a function $g$
of a small linear combination of the original variable, 
\begin{equation}
	f(\ve x) \approx g(\ma U^\trans \ve x), \qquad \ma U \in \R^{n\times m}, \quad \ma U^\trans \ma U = \ma I.
\end{equation}
Ridge functions have had great success reducing the in problems which possess an active subspace:
a low dimensional subspace of $\R^m$ along which $f$ changes~\cite{Con15}.
Although there are several classes of ridge functions $g$, % TODO Discuss later
here we choose $g$ to be a polynomial of degree $p$, $g\in \mathbb{P}^p$.
In this paper we construct an inexpensive algorithm for building 
a polynomial ridge approximation given a set of samples $\lbrace \ve x_i, f(\ve x_i)\rbrace_{i=1}^N$ 
in a least squares sense
\begin{equation}
	%\min_{\substack{g \in \mathbb{P}^p, \\ \ma U\in \R^{n\times m}, \ma U^\trans \ma U = \ma I}}
	\min_{g \in \mathbb{P}^p, \ma U \in \mathbb{G}(m, \R^n)}
		\quad \sum_{i=1}^N \left[ f(\ve x_i) - g(\ma U^\trans \ve x_i)\right]^2,	
\end{equation}
where $\mathbb{G}(m,\R^n)$ denotes the Grassmann manifold of $m$-dimensional subspaces of $\R^n$.
Our approach uses Variable Projection~\cite{GP73} implicitly solve the linear least squares problem
for the polynomial coefficients of $g$ and minimizes over $\ma U$ alone 
using Gauss-Newton method on the Grassmann manifold following Edelman, Arias, and Smith~\cite{EAS98}.
This approach offers improved performance in both speed ($4000\times$ faster) and 
accuracy (converges to machine precision) over the alternating approach
of Constantine, Eftekhari, and Ward~\cite{CEW16}.
Our faster and more accurate polynomial ridge approximation provides better surrogates,
speeds model refinement during optimization, and allows bootstrapping ridge functions.


% Motivate data-driven in sense that we only use point evaluations.
% no requirement on f -- in fact the output of f could be the result of a real experiment
% Sidesteps the curse of dimensionality, by reducing the effective dimension

The immediate advantage of ridge approximations is they combat the curse of dimensionality.


Suppose we have some quantity of interest whose value is given by the function 
$f: \set D \subset \R^m\to \R$.
Evaluating this function might take hours of computing time, if, for example,
$f$ is the thrust of a jet engine design whose evaluation requires the solution
of the Naiver-Stokes equations. 
Then, if we further seek to maximize the thrust of this engine, 
our ability to optimize will be hindered by the expense of evaluating this model.
Hence, there is a common desire to construct an inexpensive surrogate for $f$.
In this paper our goal will be to approximate $f$ by a ridge function
at a discrete set of samples in the design space $\lbrace \ve x_i \rbrace_{i=1}^N\set D$.

\hrule 

Our objective is to approximate a nonlinear scalar function $f: \set D\subseteq \R^m \to \R$
by a polynomial on a low dimensional space given samples of $f$;
i.e., given $\lbrace \ve x_i, f(\ve x_i)\rbrace_{i=1}^N$ to 
find the degree-$p$ polynomial $g\in \mathbb{P}^p$ and $m$-dimensional subspace spanned by $\ma U\in \R^{n\times m}$
such that
\begin{equation}
	f(\ve x_i) \approx g(\ma U^\trans \ve x_i), \qquad \text{where} \quad \ma U^\trans \ma U. 
\end{equation}



\hrule
 

%Given pairs of points $\ve x_i\in \set D\subset^n$ and scalar function values $f(\ve x_i)$, $f:\set D\to \R$
%our goal is to approximate 


%Response surface models are a broad class of inexpensive surrogates for expensive black box model.
%Here we develop an efficient algorithm for approximating 


A ridge function approximation mimics a nonlinear function $f: \set D \subset \R^n\to\R$
with another nonlinear function $g: \R^m\to \R$ 
whose input is an $m$-dimensional orthonormal restriction 
of the $n$-dimensional input to $f$:
\begin{equation}
	f(\ve x) \approx g(\ma U^\trans \ve x), \qquad \ma U^\trans \ma U = \ma I.
\end{equation}
Following Constantine, Eftekhari, and Ward~\cite{CEW16}
we find this ridge function approximation $\lbrace g, \ma U\rbrace$
by solving a least squares problem using $N$ samples of the map $\ve x_i \to f(\ve x_i)$ 
\begin{equation}\label{eq:opt}
	\min_{g \in \mathbb{P}^p, \ma U\in \mathbb{G}(m, \R^n)} 
		\quad \sum_{i=1}^N \left[ f(\ve x_i) - g(\ma U^\trans \ve x_i)\right]^2
\end{equation}
where $g$ is an $m$-variable polynomial of degree $p$ 
and $\ma U$ is restricted to the Grassmann manifold of $m$ dimensional subspaces of $\R^n$.
Our primary contribution is to develop a faster algorithm for solving this optimization problem.
Whereas Constantine, Eftekhari, and Ward alternate between minimizing the polynomial $g$
and the subspace $\ma U$,
we use \emph{Variable Projection}~\cite{GP73,GP03} to implicitly solve find the polynomial $g$
leaving an optimization problem over $\ma U$ alone.
This permits us to use the Gauss-Newton algorithm and obtain quadratic convergence
when the residual is small whereas the alternating minimization 
can only converge linearly~\cite{RW80}.
\jeffnote{Now we say why this is such a wonderful thing\ldots Paul, can you help?}


useful because this allows high order polynomials without hitting curse of dimensionality.


==> tab_naca.tex <==
\begin{table}
\caption{Normalized residual $\| \ve f - \ve g\|_2/\|\ve f\|_2$ where $[\ve g]_i = g(\ma U^\trans \ve x_i)$
	for $M=1756$ samples of the NACA0012 airfoil for a variety of polynomial degrees $p$ and subspace dimensions $m$.
}
\label{tab:naca}
%\begin{tabular}{cc}
%{\bf Lift} & {\bf Drag} \\
%constant: $0.48802$ & constant: $0.44815$ \\
%linear: $0.12051$ & linear : $0.17496$ \\
\begin{minipage}[t]{0.49\linewidth}
\begin{center} \bf \small Lift\end{center}
\footnotesize
constant: $0.48802$, \quad linear: $0.12051$ \\ 
\setlength\tabcolsep{5pt}
\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_naca_lift.dat}	
\end{minipage}
%&
\begin{minipage}[t]{0.49\linewidth}
\begin{center} \bf \small Drag\end{center}
\footnotesize
constant: $0.44815$, \quad linear: $0.17496$ \\ 
\setlength\tabcolsep{5pt}
\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_naca_drag.dat}	
%\end{tabular}
\end{minipage}

\end{table}


==> tab_naca_drag.tex <==
\begin{table}
	\caption{Drag Fits}
	\small
	\centering
	\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p0/.style={column name = {$p=0$}},
		columns/p1/.style={column name = {$p=1$}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p0, p1, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_naca_drag.dat}	
\end{table}


==> tab_naca_lift.tex <==
\begin{table}
	\caption{Lift Fits}
	\small
	\centering
	\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p0/.style={column name = {$p=0$}},
		columns/p1/.style={column name = {$p=1$}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p0, p1, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_naca_lift.dat}	
\end{table}


==> tab_pde.tex <==
\begin{table}
\caption{Normalized residual $\| \ve f - \ve g\|_2/\|\ve f\|_2$ where $[\ve g]_i = g(\ma U^\trans \ve x_i)$
	for $N=10^4$ samples of the elliptic PDE \cref{eq:pde} for a variety of polynomial degrees $p$ and subspace dimensions $m$.
}
\label{tab:pde}
%\begin{tabular}{cc}
%{\bf Lift} & {\bf Drag} \\
%constant: $0.48802$ & constant: $0.44815$ \\
%linear: $0.12051$ & linear : $0.17496$ \\
\begin{minipage}[t]{0.49\linewidth}
\begin{center} \bf \small Short\end{center}
\footnotesize
constant: $0.06301$, \quad linear: $0.00971$ \\ 
\setlength\tabcolsep{5pt}
\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_pde_short.dat}	
\end{minipage}
%&
\begin{minipage}[t]{0.49\linewidth}
\begin{center} \bf \small Long\end{center}
\footnotesize
constant: $0.72424$, \quad linear: $0.41477$ \\ 
\setlength\tabcolsep{5pt}
\pgfplotstabletypeset[
		clear infinite,
		fixed, fixed zerofill, precision =5,
		columns/dim/.style={int detect, column name = {dim}},
		columns/p2/.style={column name = {$p=2$}},
		columns/p3/.style={column name = {$p=3$}},
		columns/p4/.style={column name = {$p=4$}},
		columns/p5/.style={column name = {$p=5$}},
		columns = {dim, p2, p3, p4, p5},
		every head row/.style={
			before row={\toprule},
			after row={\midrule},
		},
		every last row/.style={after row=\bottomrule},
	]{fig_pde_long.dat}	
%\end{tabular}
\end{minipage}

\end{table}

